Formalization and security analysis of the Bridgeless protocol

This paper formalizes the proves the security of the Bridgeless protocol, a protocol able to bridge tokens between various chains. The Bridgeless protocol is run by a set of validators, responsible for verifying deposit transactions on the source chain and generating the corresponding withdrawals on the target chain. The protocol is designed to be chain-agnostic and the validators interact with each supported chain via a chain client. It currently supports EVM-compatible chains, the Zano, and the Bitcoin chains. The paper formalizes all involved subprotocols and describes the conditions under which the protocol maintains safety and liveness.

==> macros.tex <==
\newif\ifhide
% Enable next line to hide comments.
% \hidetrue

% \newtheorem{innercustomthm}{Theorem}
% \newenvironment{customthm}[1]
% {\renewcommand\theinnercustomthm{#1}\innercustomthm}
% {\endinnercustomthm}
%Macro for mentioning the concept of pod ( trademarked :) )1
\newcommand{\podtm}{\textsf{pod}\xspace}
\newcommand{\bidsettm}{\textsf{bidset}\xspace}
\newcommand{\bidcert}{\ensuremath{C_\text{bid}}\xspace}


\newcommand{\Ledger}{\mathbf{L}}
\newcommand{\LState}{\mathsf{L}}
\newcommand{\negl}{\textsf{negl}(\kappa)}
\newcommand{\view}{\textsc{view}}
\newcommand{\fullview}{\textsc{view}^{t,n}_{\Pi,\mathcal{A},\mathcal{Z}}}
\newcommand{\validityattack}{\textsc{persistence}\textsc{-}\textsc{game}}
\newcommand{\livenessattack}{\textsc{liveness}\textsc{-}\textsc{game}}
\newcommand{\true}{\mathsf{true}}
\newcommand{\false}{\mathsf{false}}
\newcommand{\approxn}{\widetilde{n}}
\DeclareMathOperator{\diff}{\textsf{diff}\,}
\newcommand{\dexpand}[1]{#1_{\pm\Delta}}

\newcommand{\concat}{\,\|\,}
\newcommand{\eg}{\emph{e.g., }}

\hyphenation{log-a-rith-mic}
\hyphenation{unique-ly}
\hyphenation{ex-tractabil-i-ty}

\algnewcommand\algorithmicon{\textbf{upon}}
\algblockdefx[ON]{On}{EndOn}[1]
{\algorithmicon\ #1\ \algorithmicdo}
{\algorithmicend\ \algorithmicon}

\algnewcommand\waitcommand{\textbf{wait until }}
\def\Wait#1{\State\waitcommand #1}

\def\chain{\mathcal{C}}
\DeclareMathOperator{\Ex}{\mathbb{E}}

\newcommand{\getsrandomly}{\overset{\$}{\gets}}

% Comments
\newcommand{\condtext}[1]{{\ifhide\else #1 \fi}}
\newcommand{\oa}[1]{{\color{blue}{ \condtext{OA: #1}}}}
\newcommand{\dk}[1]{{\color{red}{ \condtext{DK: #1}}}}
\newcommand{\bd}[1]{{\color{olive}{ \condtext{BD: #1}}}}
\newcommand{\wip}[1]{{\hue{WIP: #1}}}


\newcommand{\BZ}{\ensuremath{\mathbb{Z}}\xspace}
\newcommand{\CN}{\ensuremath{\mathbb{N}}\xspace}
\newcommand{\BR}{\ensuremath{\mathbb{R}}\xspace}
\newcommand{\CR}{\ensuremath{\mathcal{R}}\xspace}
\newcommand{\CL}{\ensuremath{\mathcal{L}}\xspace}
\newcommand{\CV}{\ensuremath{\mathcal{V}}\xspace}
\newcommand{\CC}{\ensuremath{\mathcal{C}}\xspace}
\newcommand{\BN}{\ensuremath{\mathbb{N}}\xspace}

\newcommand{\ceil}[1]{\lceil #1 \rceil}


%  pod
\newcommand{\op}[1]{\textsl{#1}}
\newcommand{\opwrite}[1]{\op{write(#1)}\xspace}
\newcommand{\opwriteret}[1]{\op{write\_return(#1)}\xspace}
\newcommand{\opwritedeps}[1]{\op{store(#1)}\xspace}
\newcommand{\opread}[1]{\op{read(#1)}\xspace}
\newcommand{\opreadall}[1]{\op{read(#1)}\xspace}
\newcommand{\opreadallret}[1]{\op{read\_return(#1)}\xspace}
\newcommand{\opgetdeps}[1]{\op{get\_deps(#1)}\xspace}
\newcommand{\opbcast}[1]{\op{broadcast(#1)}\xspace}
\newcommand{\opdel}[1]{\op{deliver(#1)}\xspace}
\newcommand{\opSign}[1]{\ensuremath{\op{Sign(#1)}\xspace}}
\newcommand{\opVerify}[1]{\op{Verify(#1)}\xspace}
\newcommand{\opmin}[1]{\op{min(#1)}\xspace}
\newcommand{\opmax}[1]{\op{max(#1)}\xspace}
\newcommand{\opmed}[1]{\op{med(#1)}\xspace}
\newcommand{\opvalid}[1]{\op{valid(#1)}\xspace}
\newcommand{\opdisperse}[1]{\op{disperse(#1)}\xspace}
\newcommand{\opretrieve}[1]{\op{retrieve(#1)}\xspace}
\newcommand{\opOnReceiveVote}[1]{\op{handleVote(#1)}\xspace}
\newcommand{\opOnReceiveHeartBeat}[1]{\op{handleHeartBeat(#1)}\xspace}
\newcommand{\opSendVote}[1]{\op{doVote(#1)}\xspace}
\newcommand{\opMinPossibleTs}[1]{\op{minPossibleTs(#1)}\xspace}
\newcommand{\opMaxPossibleTs}[1]{\op{maxPossibleTs(#1)}\xspace}
\newcommand{\opMinPossibleTsForNewTx}[1]{\op{minPossibleTsForNewTx(#1)}\xspace}
\newcommand{\opMed}[1]{\op{median(#1)}\xspace}
\newcommand{\opInit}[1]{\op{init(#1)}\xspace}
\newcommand{\opTime}{\op{round()}\xspace}
\newcommand{\opAppend}[1]{\op{append(#1)}\xspace}
\newcommand{\opKeys}{\op{keys()}\xspace}
\newcommand{\opValues}{\op{values()}\xspace}
\newcommand{\opAccountableFault}[1]{\op{AccountableFault}(#1)\xspace}
\newcommand{\opHash}[1]{\op{hash(#1)}\xspace}

\newcommand{\operand}[1]{\textsf{#1}}
\newcommand{\tx}{\operand{tx}\xspace}
\newcommand{\deptx}{\operand{deptx}\xspace}
\newcommand{\deptxid}{\operand{txid}\xspace}
\newcommand{\txid}{\operand{txid}\xspace}
\newcommand{\round}{\operand{r}\xspace}
\newcommand{\client}{\operand{c}\xspace}
\newcommand{\sk}{\operand{sk}\xspace}
\newcommand{\pk}{\operand{pk}\xspace}

\newcommand{\var}[1]{\operand{#1}}
\newcommand{\const}[1]{\textsc{#1}}
\newcommand{\type}[1]{\textit{#1}}
\newcommand{\event}[1]{\textsc{#1}}

\newcommand{\heartBeat}{\textsc{heartBeat}\xspace}

\newcommand{\rexp}{\ensuremath{\round_\text{exp}}\xspace}
\newcommand{\rconf}{\ensuremath{\round_\text{conf}}\xspace}
\newcommand{\rmin}{\ensuremath{\round_\text{min}}\xspace}
\newcommand{\rmax}{\ensuremath{\round_\text{max}}\xspace}
\newcommand{\rinterval}{\ensuremath{[\rmin, \rmax]}\xspace}
\newcommand{\rreported}{\ensuremath{\round_\text{rep}}\xspace}
\newcommand{\rperf}{\ensuremath{\round_\text{perf}}\xspace}
\newcommand{\rloc}{\ensuremath{\round_\text{loc}}\xspace}
\newcommand{\txmiss}{\ensuremath{\txset_\text{miss}}\xspace}
\newcommand{\txfinal}{\ensuremath{\txset_\text{final}}\xspace}
\newcommand{\inclist}{\ensuremath{L}\xspace}
\newcommand{\rep}{\ensuremath{R}\xspace}
\newcommand{\allreps}{\CR}
\newcommand{\allClients}{\CC}
\newcommand{\mrt}{\operand{mrt}\xspace}
\newcommand{\repLog}{\operand{replicaLog}\xspace}
\newcommand{\opGetVote}{\op{getVoteMsg()}\xspace}
\newcommand{\vote}{\operand{vote}\xspace}
\newcommand{\sendHeartBeat}{\operand{sendHeartBeat}\xspace}
\newcommand{\transactions}{\operand{\wip{obsolete}}\xspace}
\newcommand{\allTxs}{\operand{T}\xspace}
\newcommand{\tsps}{\operand{tsps}\xspace}
\newcommand{\sigs}{\operand{sigs}\xspace}
\newcommand{\txVotesMin}{\operand{timestamps}\xspace}
\newcommand{\txVotesMax}{\operand{timestamps}\xspace}
\newcommand{\txVotesPerf}{\operand{timestamps}\xspace}
\newcommand{\txVotes}{\operand{timestamps}\xspace}
\newcommand{\certSize}{\ensuremath{c}\xspace}
\newcommand{\tsp}{\operand{ts}\xspace}
\newcommand{\opGetVotedReplicas}{\operand{votedReplicas}\xspace}
\newcommand{\missingReplicas}{\operand{missingReplicas}\xspace}
\newcommand{\opnext}{\operand{next\_message}\xspace}
\newcommand{\nextmsg}{\operand{msg}\xspace}
\newcommand{\state}{\operand{state}\xspace}
\newcommand{\req}{\operand{request}\xspace}


\newcommand{\replicas}{\ensuremath{R}\xspace}
\newcommand{\cheaters}{\ensuremath{\tilde{\replicas}}\xspace}
\newcommand{\identify}[1]{\ensuremath{\mathsf{identify}(#1)}\xspace}
\newcommand{\identifyAuctioneer}[1]{\ensuremath{\mathsf{identifyAuctioneer}(#1)}\xspace}


\newcommand{\user}{\operand{user}\xspace}
\newcommand{\timestamp}{\operand{ts}\xspace}
\newcommand{\txcert}{\ensuremath{C_\text{tx}}\xspace}
\newcommand{\ppcert}{\ensuremath{C_\text{pp}}\xspace}
\newcommand{\txSet}{\operand{T}\xspace}
\newcommand{\final}{\operand{f}\xspace}
\newcommand{\parConf}{\ensuremath{u}\xspace}
\newcommand{\parLive}{\ensuremath{v}\xspace}
\newcommand{\parPerf}{\ensuremath{w}\xspace}
\newcommand{\parTemp}{\ensuremath{\theta}\xspace}
\newcommand{\parAuctionTerm}{\ensuremath{W}\xspace}
\newcommand{\tProp}{\ensuremath{t_\text{prop}}\xspace}
\newcommand{\parAgr}{\ensuremath{z}\xspace}
\newcommand{\Pod}{\ensuremath{D}\xspace}
\newcommand{\limbo}{\ensuremath{L}\xspace}
\newcommand{\podView}[2]{\ensuremath{\Pod_{#2}^{#1}}\xspace}
\newcommand{\tran}{\ensuremath{T}\xspace}

\newcommand{\dotparagraph}[1]{\paragraph*{#1.}}

\newcommand{\returns}{\ensuremath{\rightarrow}\xspace}
% \newcommand{\dotparagraph}[1]{\paragraph*{\textbf{#1.}}}
\newcommand{\confirmed}{confirmed\xspace}
\newcommand{\Confirmed}{Confirmed\xspace}
\newcommand{\finalized}{finalized\xspace}
\newcommand{\pend}{pending-confirmation\xspace}
\newcommand{\ispend}{\ensuremath{\text{is\_pend}}\xspace}
\newcommand{\zo}{\ensuremath{\{ 0, 1\}\xspace}}

% for pseudocode
\newcommand{\return}[1]{\State{\textbf{return} #1}\xspace}
\newcommand{\st}{\textbf{such that}\xspace}
\newcommand{\andl}{\textbf{and}\xspace}
\newcommand{\msg}[2]{\ensuremath{\langle\textit{\uppercase{#1 }}#2\rangle}\xspace}
\newcommand{\msgwrite}[1]{\msg{write}{ #1}}
\newcommand{\msgwriteresp}[1]{\msg{write-resp}{ (#1)}}
\newcommand{\msgread}[1]{\msg{read}{#1}}
\newcommand{\msgreadresp}[1]{\msg{read-resp}{ #1}}
\newcommand{\msgconnect}{\msg{connect}{}}
\newcommand{\msgrecord}[1]{\msg{vote}{ #1}}
\newcommand{\msgbidresult}[1]{\msg{bids}{ #1}}
\newcommand{\msgproposal}[1]{\msg{proposal}{(#1)}}
\newcommand{\msgacceptance}[1]{\msg{acceptance}{ (#1)}}
\newcommand{\msgsignstart}[1]{\msg{signStart}{ (#1)}}
\newcommand{\msgproposalEMPTY}{\msg{proposal}{}}
\newcommand{\msgacceptanceEMPTY}{\msg{acceptance}{}}
\newcommand{\msgsignstartEMPTY}{\msg{signStart}{}}
\newcommand{\msgsubmitwithrawal}[1]{\msg{submit-withdrawal}{ #1}}
\newcommand{\msgcheckwithrawal}[1]{\msg{check-withdrawal}{ #1}}
\newcommand{\msgcheckwithrawalEMPTY}[1]{\msg{check-withdrawal}{}}
\newcommand{\msgcheckwithrawalresponse}[1]{\msg{check-response}{ #1}}


\newcommand{\Guard}[1]{\State{\textbf{require }\ensuremath{#1}\xspace}}
\newcommand{\error}{\const{Error}\xspace}



\let\oldalpha\alpha
\renewcommand{\alpha}{\ensuremath{\oldalpha}\xspace}
\let\oldbeta\beta
\renewcommand{\beta}{\ensuremath{\oldbeta}\xspace}

% auction
\newcommand{\tzero}{\ensuremath{t_0}\xspace}
\newcommand{\tone}{\ensuremath{t_1}\xspace}
\newcommand{\ttwo}{\ensuremath{t_2}\xspace}
\newcommand{\tthree}{\ensuremath{t_3}\xspace}
\newcommand{\tfour}{\ensuremath{t_4}\xspace}
\newcommand{\auc}{\ensuremath{a}\xspace}
\newcommand{\bag}{\ensuremath{B}\xspace}
\newcommand{\opresult}[1]{\op{result(#1)}\xspace}
\newcommand{\mes}{\ensuremath{m}\xspace}
\newcommand{\sig}{\ensuremath{\sigma}\xspace}
\newcommand{\opBid}[1]{\op{bid(#1)}\xspace}
\newcommand{\opResult}[1]{\op{result(#1)}\xspace}
\newcommand{\opSubmitBid}[1]{\op{submitBid(#1)}\xspace}
\newcommand{\opRunAuction}[1]{\op{readBids(#1)}\xspace}
\newcommand{\opReadResult}[1]{\op{readResult(#1)}\xspace}
\newcommand{\bid}{\ensuremath{b}\xspace}
\newcommand{\podInst}{\textit{pod}\xspace}

\newcommand{\etal}{\textit{et~al.}\@}

\newcommand{\ewnp}{except with negligible probability\xspace}

\newcommand{\sn}{\operand{sn}\xspace}
\newcommand{\nextsn}{\operand{nextsn}\xspace}

% This is a solution to support adding links within floats (pseudocode)
% Use \goto{} inside the float to put the marker.
% Use \codelink{<LINK>} outside the float to put the link.
% For the link counters to work correctly, the code must use
\newcounter{linkcounter}
\setcounter{linkcounter}{1}
\newcounter{gotocounter}
\setcounter{gotocounter}{1}
\newcommand{\goto}{
  {\textsuperscript{\thegotocounter}}
  \stepcounter{gotocounter}
}
\newcommand{\codelink}[1]{{% Group to localize change to footnote
\renewcommand{\thefootnote}{\thelinkcounter}% Update footnote counter representation
  \footnotetext[0]{\url{#1}}}% Print footnote text
  \stepcounter{linkcounter}
}

\newcommand{\ChainClient}{\var{ChainClient}\xspace}
\newcommand{\sourceClient}{\var{sourceClient}\xspace}
\newcommand{\targetClient}{\var{targetClient}\xspace}
\newcommand{\emptyString}{\ensuremath{\bot}\xspace}

\newcommand{\btm}{\textsf{Bridgeless}\xspace}
\newcommand{\varIsWrapped}{}



==> sections/chain-client-zano.tex <==

\section{The chain client for Zano}

\input{pseudocode/chain-client-zano.tex}

The \ChainClient for Zano, shown in \Cref{alg:zano-chain-client}, works similar to the one for EVM.
The validator maintains an RPC client to the Zano chain \oa{Add information: who runs it, what trust assumptions}, which they use to retrieve the deposit transaction (\cref{line:zano-get-transaction}) and extract the required fields (lines \ref{line:zano-extract-begin}--\ref{line:zano-extract-end}) to form a \type{DepositData} (\cref{line:zano-return-deposit-data}).


